Random Quadratic Forms with Dependence: Applications to Restricted Isometry and Beyond

Several important families of computational and statistical results in machine learning and randomized algorithms rely on uniform bounds on quadratic forms of random vectors or matrices. Such results include the Johnson-Lindenstrauss (J-L) Lemma, the Restricted Isometry Property (RIP), randomized sketching algorithms, and approximate linear algebra. The existing results critically depend on statistical independence, e.g., independent entries for random vectors, independent rows for random matrices, etc., which prevent their usage in dependent or adaptive modeling settings. In this paper, we show that such independence is in fact not needed for such results which continue to hold under fairly general dependence structures. In particular, we present uniform bounds on random quadratic forms of stochastic processes which are conditionally independent and sub-Gaussian given another (latent) process. Our setup allows general dependencies of the stochastic process on the history of the latent process and the latent process to be influenced by realizations of the stochastic process. The results are thus applicable to adaptive modeling settings and also allows for sequential design of random vectors and matrices. We also discuss stochastic process based forms of J-L, RIP, and sketching, to illustrate the generality of the results.

==> app/azuma.tex <==
\section{The Azuma-Hoeffding Inequality}
A sequence of random variables $Z_1,Z_2,\ldots$, is called a {\em martingale difference sequence} (MDS) with respect to another sequence of random variables $X_1,X_2,\ldots$, if for any $t$, $E[|Z_{t}|] < \infty$ and $E[Z_{t}|X_1, \ldots,X_{t-1}] = 0$ almost surely. By construction, if $X_t$ is a martingale, then $Z_{t} = X_{t} - X_{t-1}$ will be a MDS, which explains the name.


Let $\{X_t, t=0,1,2,\ldots \}$ be a martingale sequence, and let $Z_t = X_t - X_{t-1}$ be a MDS. Assume that $Z_t$ is bounded, i.e.,
\beq
|Z_t| = |X_t - X_{t-1}| < c_t~,
\eeq
and let $\c = [c_1 ~\ldots ~ c_T]$ be the vector of the upper bounds. Then, the Azuma-Hoeffding inequality states that: for any $\tau > 0$,
\beq
P \left( \left|\sum_{t=1}^T Z_t \right| \geq \tau \right) \leq 2 \exp \left\{ -\frac{\tau^2}{2\|\c\|_2^2} \right\}~.
\eeq
For the special case when $c_t = c$, the bound can be simplified to: for any $\epsilon > 0$
\beq
P \left( \frac{1}{T} \left|\sum_{t=1}^T Z_t \right| \geq \epsilon \right) \leq 2 \exp \left\{ - T \frac{\epsilon^2}{2c^2} \right\}~.
\eeq
The result can be extended to the setting of general subGaussian tails for $Z_t$, e.g., see~\cite{sham11}, and also applies to general MDSs $Z_t|\cF_{t-1}$ where $\{\cF_t\}$ is the filtration.

\section{The Azuma-Bernstein Inequality}
Let $\{X_t, t=0,1,2,\ldots \}$ be a martingale sequence, and let $Z_t = X_t - X_{t-1}$ be a MDS. However, we now assume that $Z_t|X_1,\ldots,X_{t-1}$ has a sub-exponential tail, so that
\beq
P( |Z_t|X_1,\ldots,X_{t-1}| \geq \tau ) \leq 2 \exp(-c \tau/\kappa)~,
\label{eq:subexp}
\eeq
where $\kappa = \vertiii{Z_t|X_1,\ldots,X_{t-1}}_{\psi_1}$ is the sub-exponential norm or $\psi_1$ norm~\cite{vers12}. Then, we have the following result:
\begin{theo}
Let $\{Z_t\}$ be a MDS which satisfies \myref{eq:subexp}. Then, for every $\a = [a_1~\ldots~a_T] \in \R^T$, for any $\tau > 0$, we have
\beq
P \left( \left|\sum_{t=1}^T a_t Z_t \right| \geq \tau \right) \leq 2 \exp \left\{ - \min\left( \frac{\tau^2}{4c\kappa^2 \|\a\|_2^2},\frac{\eta \tau}{2\kappa \|\a\|_{\infty}} \right) \right\}~,
\label{eq:ab1}
\eeq
for absolute constants $c,\eta > 0$. In particular, for any $\epsilon > 0$, for a constant $\gamma > 0$, we have
\beq
P \left( \frac{1}{T} \left|\sum_{t=1}^T Z_t \right| \geq \epsilon \right) \leq 2 \exp \left\{ - \gamma T \min\left( \frac{\epsilon^2}{\kappa^2},\frac{\epsilon}{\kappa} \right) \right\}~.
\label{eq:ab2}
\eeq
\end{theo}
\proof Recall that if $Y$ is a sub-exponential random variable, then the moment-generating function (MGF) of $Y$ satisfies the following result \cite[Lemma 5.15]{vers12}: For $s$ such that $|s| \leq \eta/\kappa_1$, we have
\beq
E[\exp(sY)] \leq \exp(c s^2 \kappa^2)~,
\label{eq:mgf1}
\eeq
where $\kappa_1 = \vertiii{Y}_{\psi_1}$ and $\eta,c$ are absolute constants. In particular, since $Z_t|{\cal F}_{t-1}$ are subexponential, with $\kappa_1 = \max_t \vertiii{Z_t|X_1,\ldots,X_{t-1}}_{\psi_1}$, for $|s| \leq \eta/\kappa_1$, we have
\beq
E_{X_t|X_1,\ldots,X_{t-1}}[\exp(s Z_t)] \leq \exp(c s^2 \kappa_1^2)~,\quad \forall t~.
\label{eq:mgf2}
\eeq
For any $s > 0$, note that
\beq
P \left( \sum_{t=1}^T a_t Z_t \geq \tau \right) = P\left( \exp\left( s\sum_{t=1}^T a_t Z_t \right) \geq \exp(s\tau) \right) \leq \exp(-s \tau) E\left[ \exp\left( s\sum_{t=1}^T a_t Z_t \right) \right]~.
\label{eq:bnd1}
\eeq
For $|s| \leq \eta/(\kappa_1 \| \a \|_{\infty})$ so that $|a_t s| \leq \eta/\kappa_1$ for all $t$, the expectation can be bounded using~\myref{eq:mgf2} as follows:
\begin{align*}
E&\left[ \exp\left( s\sum_{t=1}^T a_t Z_t \right) \right] = E_{(X_1,\ldots,X_T)}\left[ \prod_{t=1}^T \exp (s a_t Z_t) \right]\\
&= E_{(X_1,\ldots,X_{T-1})}\left[ E_{X_T|X_1,\ldots,X_{T-1}}\left[ \exp( s a_T Z_T )\right] \prod_{t=1}^{T-1} \exp (s a_t Z_t) \right]~\\
& \leq \exp( c s^2 a_T^2 \kappa^2) E_{(X_1,\ldots,X_{T-1})}\left[ \prod_{t=1}^{T-1} \exp (s a_t Z_t) \right]\\
& \leq  \exp( c s^2 a_T^2 \kappa^2) \exp(c s^2 a_{T-1}^2 \kappa^2) E_{(X_1,\ldots,X_{T-2})}\left[ \prod_{t=1}^{T-2} \exp (s a_t Z_t) \right] \\
& \cdots \\
& \leq \exp\left( c s^2 \kappa^2 \| \a\|_2^2 \right)~.
\end{align*}
Plugging this back to \myref{eq:bnd1}, for $|s| \leq \eta/\kappa$, we have
\begin{align}
P & \left( \sum_{t=1}^T a_t Z_t \geq \tau \right) \leq \exp(-s \tau + c s^2 \kappa^2 \|\a\|_2^2 )~.
\end{align}
Choosing $s = \min\left( \frac{\tau}{2c \kappa^2 \|\a\|_2^2}, \frac{\eta}{\kappa\|\a\|_{\infty}} \right)$, we obtain \beq
P \left( \sum_{t=1}^T a_t Z_t \geq \tau \right) \leq \exp \left\{ - \min \left( \frac{\tau^2}{4c\kappa^2 \|\a\|_2^2}, \frac{\eta \tau}{2\kappa \|\a\|_{\infty}} \right) \right\}~.
\eeq
Repeating the same argument with $-Z_t$ instead of $X_t$, we obtain the same bound for $P( - \sum_t a_t Z_t \geq \tau)$. Combining the two results gives us \myref{eq:ab1}.

Now, with $a_t = 1, t=1,\ldots,T$, and $\tau = T \epsilon$ in \myref{eq:ab1}, for a suitable constant $\gamma > 0$ we have
\beq
P \left( \frac{1}{T} \left| \sum_{t=1}^T Z_t \right| \geq \epsilon \right) \leq \exp \left\{ - \gamma T \min \left( \frac{\epsilon^2}{\kappa^2}, \frac{\epsilon}{\kappa} \right) \right\}~.
\eeq
That completes the proof. \qed

The result can also be stated in terms of a general sub-exponential MDS $Z_t|\cF_{t-1}$, where $\{ \cF_t\}$ is the filtration.

% \section{Elementwise Concentration for Martingale Designs}
% We will shamelessly abuse notation to get started on the smoothed bandit analysis. Let $[T]$ denote $1,\ldots,T$.

% Let $X_T \in \R^{T \times p}$ be a {\em martingale design} matrix, with rows $\x_t \in \R^p, t \in [T]$. Let $\u \in S^{p-1}$ be any fixed unit vector. Consider the sequence $Z_t = \langle \x_t, \u \rangle, t \in [T]$.
% We say the design $X_T$ is a {\em martingale design} if the sequence $\{Z_t\}$ is a MDS.

% For a fixed $\u \in S^{p-1}$, consider the stochastic process {\em indexed by $\u$}: $Y_u =  \frac{1}{T} \| X_T \u \|_2^2$. We should denote the process as $Y_{u,T}$ to indicate the dependence on $T$, but the
% exact same analysis will hold for any $T$, so we are dropping the subscript $T$ to keep the notation simple. We first establish a large deviation bound for $Y_u$ around its expectation $E[Y_u]$, where the expectation is over the randomness in the martingale design matrix $X_T$.

% Let $Z_t = \langle \x_t, \u \rangle$. Based on our assumptions, $Z_t$ is a univariate sub-Gaussian MDS. Let $\cF_{t-1}$ denote the filtration till $(t-1)$ so that $E[Z_t|\cF_{t-1}] = 0$.
% Let $\mu_t = E[Z_t^2|\cF_{t-1}]$, where we note that $\mu_t$ will in fact depend on $\u$. Further, let $\| Z_t | \cF_{t-1} \|_{\psi_2} \leq \kappa_2$. Then, $(Z_t^2 - \mu_t)|\cF_{t-1}$ is a zero mean sub-exponential
% MDS with $\| Z_t^2 - \mu_t |\cF_{t-1} \|_{\psi_1} \leq \kappa_1$. Then,
% \begin{equation}
% P\left[ | Y_u - E[Y_u] | \geq \epsilon \right] = P\left[ \left| \frac{1}{T} \sum_{t=1}^T (Z_t^2 - \mu_t) \right| \geq \epsilon \right]
%  \stackrel{(a)}{\leq} 2 \exp \left\{ -\gamma T \min \left( \frac{\epsilon^2}{\kappa^2}, \frac{\epsilon}{\kappa} \right) \right\}~
% \end{equation}
% where (a) follows by the Azuma-Bernstein bound.

% We may also be able to get a bound on the process $\sqrt{Y_u} - E[\sqrt{Y_u}]$ of the form
% \begin{equation}
% P\left[ | \sqrt{Y_u} - E[\sqrt{Y_u}] | \geq \epsilon \right] \leq 2 \exp \left\{ - \frac{\gamma T \epsilon^2}{\kappa^2} \right\}~
% \label{eq:u_sqrt}
% \end{equation}
% using Azuma-Hoeffding.


==> sec/gen-diag-bnd.tex <==
For the diagonal terms corresponding to bounded random variables, we have the following main result:
\begin{theo}
Let $\cA \in \R^{m \times n}$ be a collection of $(m \times n)$ matrices. $\xi_1,\ldots,\xi_n$ be a bounded MDS, and let $\bxi \in \R^n$
denote a vector of these random variables. Consider the random variable
\begin{equation}
    D_{\cA}(\bxi) = \sup_{A \in \cA} \left| \sum_{j=1}^n ( \xi_j^2 - E|\xi_j|^2 ) \| A^j \|_2^2 \right|~,
\end{equation}
where $A^j$ denotes the $j^{th}$ column of $A$. Then, we have 
\begin{equation}
    \| D_{\cA}(\xi) \|_{L_p} \leq  d_F(\cA) \cdot \gamma_2(  \cA, \| \cdot \|_{2 \rightarrow 2} ) + \sqrt{p} \cdot d_F(\cA) \cdot d_{2 \rightarrow  2} (\cA)~.
\end{equation}
\label{theo:subg-diag-bnd}
\end{theo}

The main observation here is since $\xi_j$ are bounded, so are $\xi_j^2$, implying $\eta = \xi_j^2 - E|\xi_j|^2$ is also sub-Gaussian, and the sequence $\eta_1,\ldots,\eta_n$ is a sub-Gaussian MDS~\cite{vers14}. Based on this observation, the proof of Theorem~\ref{theo:subg-diag-bnd} relies on the following result bounding $L_p$-norms of the supremum of sub-Gaussian MDSs:
\begin{lemm}
    Let $\bzeta = [\zeta_1,\ldots,\zeta_n]$ be a $L$-sub-Gaussian MDS and let $T \in \R^n$. Then, for every $p \geq 1$,
    \begin{align}
        \left( E \sup_{t \in T} | \langle t, \bzeta \rangle |^p \right)^{1/p} & \leq c_2 \left( E \left[ \sup_{t \in T} | \langle t, \bgg \rangle | \right] + \sup_{t \in T} \left( E| \langle t, \bzeta \rangle|^p \right)^{1/p} \right)~ 
    \end{align}
    where $c_2$ is a constant which depends on $L$, $\bgg = [g_j]$ where $g_j \sim N(0,1)$ are independent identically distributed normal random variables.
%    $\eta = [\eta_j]$ where $\eta_j$ are independent identically distributed exponential random variables.
    % \begin{align}
    %     \left( E \sup_{t \in T} | \langle t, \bzeta \rangle |^p \right)^{1/p} & \leq c_2 \left( E \left[ \sup_{t \in T} | \langle t, \bgg \rangle | \right] + E \left[ \sup_{t \in T} | \langle t, \beeta \rangle | \right] + \sup_{t \in T} \left( E| \langle t, \bzeta \rangle|^p \right)^{1/p} \right)~ 
    % \end{align}(a)
    % where $c_2$ is a constant which depends on $L$, $\bgg = [g_j]$ where $g_j$ are independent identically distributed normal random variables, and
    % $\eta = [\eta_j]$ where $\eta_j$ are independent identically distributed exponential random variables.
\label{lemm:lpnormg2}
\end{lemm}
\proof We assume $T$ is finite without loss of generality. Let $\{T_r\}$ be an optimal admissible sequence of $T$. For any $t \in T$, let $\pi_r(t) = \argmin_{t_r \in T_r} \| t - t_r\|_2$. For any given $p$ determining the $p$-norm, choose $\ell$ such that $2^{\ell-1} \leq 2p \leq 2^{\ell}$, so that $2^{\ell} / p \leq 4$. Then, by triangle inequality, we have
\begin{equation}
    \sup_{t \in T}|\langle t,\bzeta \rangle| \leq \sup_{t \in T} | \langle \pi_{\ell}(t), \bzeta \rangle | + \sup_{t\in T} \sum_{r=\ell}^{\infty} | \langle \pi_{r+1}(t) - \pi_r(t), \bzeta \rangle |~.
\end{equation}
For the first term, note that
\begin{align*}
    \left( E \sup_{t \in T} | \langle \pi_{\ell}(t), \bzeta \rangle |^p \right)^{1/p} 
    & \leq \left( E \sum_{t \in T_{\ell}} | \langle t, \bzeta \rangle |^p \right)^{1/p} \\
    & \leq (|T_{\ell}|)^{1/p} \sup_{t \in T_{\ell}} \left(E| \langle t, \bzeta \rangle |^p \right)^{1/p} \\
    & \leq (2^{2^{\ell}})^{1/p} \sup_{t \in T} (E|\langle t,\bzeta \rangle|^p)^{1/p} \\
    & \leq 16 \sup_{t \in T} (E|\langle t,\bzeta \rangle|^p)^{1/p}~.
\end{align*}
% we first define the following function:
% \begin{align}
%     f(u, r, t, t', \{x_j\}) = \begin{cases}
%     u L_2 2^{r/2} \| (\langle \pi_{r+1}(t) - \pi_r(t), x_j \rangle)_{j=1}^n \|_2~, & ~~\text{if}~~ u \leq L_2^2/L_1~, \\
%     u L_{\infty} 2^{r} \| (\langle \pi_{r+1}(t) - \pi_r(t), x_j \rangle)_{j=1}^n \|_{\infty}~, & ~~ \text{otherwise}~.
%     \end{cases}
% \end{align}
For the second term, for any $u \geq 0$, we have 
\begin{align*}
    P & \bigg( \sup_{t\in T} \sum_{r=\ell}^{\infty} | \langle \pi_{r+1}(t) - \pi_r(t), \bzeta \rangle | 
    \geq  u L 2^{r/2} \|  \pi_{r+1}(t) - \pi_r(t) \|_2   \bigg)  \\
    & \leq \sum_{t=\ell}^{\infty} \sum_{t \in T_{r+1}} \sum_{t' \in T_r} P \bigg( \bigg| \langle t - t', \bzeta \rangle \bigg| \geq u L 2^{r/2} \| t - t' \|_2 \bigg) \\
    & \stackrel{(a)}{\leq} \sum_{r=\ell}^{\infty} 2^{2^{r+1}} \cdot 2^{2^r} \cdot \exp (-2^{r} u^2) 
    \leq 2 \exp(- 2^{\ell} u^2) \\
    & \leq 2 \exp(-p u^2)~,
\end{align*}
for $u \geq u_0$, a constant, and where (a) follows from the Azuma-Hoeffding inequality. 

Then, from Proposition~\ref{prop:subg}, we have
\begin{align*}
    \left( E \sup_{t\in T} \sum_{r=\ell}^{\infty} | \langle \pi_{r+1}(t) - \pi_r(t), \bzeta \rangle |^p \right)^{1/p} 
    & \leq L \sum_{r=\ell}^{\infty} \bigg( 2^{r/2} \| \pi_{r+1}(t) - \pi_r(t) \|_2 \bigg)  \leq L \gamma_2(T, \| \cdot \|_2) ~.
\end{align*}
% where $T' = \{ (\langle t, x_j \rangle)_{j=1}^n | t \in T \}$. 
Then, by the majorizing measures theorem [][], we have
\begin{equation*}
     \gamma_2(T,\| \cdot \|_2 ) \leq E \sup_{t \in T} |  \langle t, \bgg \rangle |~,
\end{equation*}
where $\bgg = [g_j], g_j \sim N(0,1)$. That completes the proof. \qed


%\ab{Proof of Theorem~\ref{theo:subg-diag} can be now be done using Lemma~\ref{lemm:lpnorme}.}

{\em Proof of Theorem~\ref{theo:subg-diag-bnd}.} Consider the random variable $\bzeta^{(A)} = \sum_{j=1}^n (\xi^2 - E|\xi_j|^2) \| A^j \|_2^2$. Then, for any $A,B \in \cA$, by Azuma-Hoeffding inequality, we have
\begin{equation}
    P\left( | \bzeta^{(A)} - \bzeta^{(B)} | \geq \eps\right) \leq 2 \exp \left\{ - \frac{\eps^2}{d_2^2(A,B)} \right\}~, 
\end{equation}
where
\begin{align*}
    d_2(A,B) &= ~ \left( \sum_{j=1}^n (\| A^j \|_2^2 - \| B^j \|_2^2 )^2 \right)^{1/2} \\ 
    & = ~ \left( \sum_{j=1}^n ( \| A^j \|_2 - \| B^j \|_2 )^2 \cdot (\| A^j \|_2 + \| B^j \|_2 )^2 \right)^{1/2} \\
    & \stackrel{(a)}{\leq} ~ \left( \sum_{j=1}^n \| A^j - B^j \|_2^2 \cdot (\| A^j \|_2 + \| B^j \|_2 )^2 \right)^{1/2} \\
    & \leq ~ 2 d_F(\cA) \| A - B \|_{2 \rightarrow 2}~,
\end{align*}
where (a) follows from triangle inequality. From the majorizing measure theorem~\cite{tala14} we have
$E[\sup_{t \in T}|\langle t, \bgg \rangle|] \leq \gamma_2(T, d_2)$.
Then, from Lemma~\ref{lemm:lpnormg2} and Proposition~\ref{prop:subg}, we have
\begin{align*}
 \| D_{\cA}(\bxi) \|_{L_p} 
  & \leq  d_F(\cA) \cdot \gamma_2(  \cA, \| \cdot \|_{2 \rightarrow 2} ) + \sqrt{p} \cdot d_F(\cA) \cdot d_{2 \rightarrow  2}(\cA) ~.
\end{align*}
That completes the proof. \qed



==> sec/gen-diag.tex <==
For the diagonal terms corresponding to unbounded sub-Gaussian random variables, we have the following main result:
\begin{theo}
Let $\cA \in \R^{m \times n}$ be a collection of $(m \times n)$ matrices. $\xi_1,\ldots,\xi_n$ be a sub-Gaussian MDS, and let $\xi \in \R^n$
denote a vector of these random variables. Consider the random variable
\begin{equation}
    D_{\cA}(\xi) = \sup_{A \in \cA} \left| \sum_{j=1}^n ( \xi_j^2 - E|\xi_j|^2 ) \| A^j \|_2^2 \right|~,
\end{equation}
where $A^j$ denotes the $j^{th}$ column of $A$. Then, we have 
% \begin{equation}
% \begin{split}
%     \| D_{\cA}(\xi) \|_{L_p} \leq &~ \gamma_{2 \rightarrow 2}(\cA, \| \cdot \|_{2 \rightarrow 2}) ~ [ \gamma_2(\cA, \| \cdot \|_{2 \rightarrow 2}) + d_F(\cA)] \\
%     & + \sqrt{p} \cdot d_{2 \rightarrow 2}(\cA) ~ [ \gamma_2(\cA, \| \cdot \|_{2 \rightarrow 2}) + d_F(\cA)] \\
%     & + p \cdot d_{2 \rightarrow 2}^2(\cA)~.
% \end{split}
% \end{equation}
\begin{equation}
    \| D_{\cA}(\xi) \|_{L_p} \leq  \sqrt{\log n} 
    \cdot d_F(\cA) \cdot \gamma_2(  \cA, \| \cdot \|_{2 \rightarrow 2} ) + \sqrt{p} \cdot d_F(\cA) \cdot d_{2 \rightarrow  2} (\cA) + p \cdot d_F(\cA) \cdot d_{2,\infty}(\cA)~.
%    \| D_{\cA}(\xi) \|_{L_p} \leq &~ \sqrt{\log n} \cdot \gamma_2(\cA, \| \cdot \|_{F}) +  \sqrt{p} \cdot d_F(\cA) + p \cdot d_{2,\infty}(\cA)~.
\end{equation}
\label{theo:subg-diag}
\end{theo}

%where (a) follows from Theorem~\ref{theo:exp-width} and (b) follows from the majorizing measures theorem [][]. Further, from Proposition~\ref{prop:sube2}, we have 

%\ab{Note that the bound can be stated in the $(a + \sqrt{p} \cdot b + p \cdot p)$ form using the upper bound on $\| N_{\cA} \|_{L_p}$ from Lemma~\ref{lemm:scaling}.}

The proof of Theorem~\ref{theo:subg-diag} relies on the following result bounding $L_p$-norms of the supremum of sub-exponential MDS processes:
% \begin{lemm}
%     Let $x_1,\ldots,x_n \in \R^d$ and $T  \subset \R^d$. Let $\xi_1,\ldots,\xi_n$ be a $L$-sub-exponential MDS and let $y = \sum_{j=1}^n \xi_j x_j$. Then, for every $p \geq 1$,
%     \begin{align}
%         \left( E \sup_{t \in T} | \langle t, \bzeta \rangle |^p \right)^{1/p} & \leq c_2 \left( E \left[ \sup_{t \in T} | \langle t, g \rangle | \right] + E \left[ \sup_{t \in T} | \langle t, \eta \rangle | \right] + \sup_{t \in T} \left( E| \langle t, \bzeta \rangle|^p \right)^{1/p} \right)~ 
%     \end{align}
%     where $c_2$ is a constant which depends on $L$, $g = \sum_{j=1}^n g_j x_j$ where $g_j$ are independent identically distributed normal random variables, and
%     $\eta = \sum_{j=1}^n \eta_j x_j$ where $\eta_i$ are independent identically distributed exponential random variables.
% \label{lemm:lpnorme}
% \end{lemm}
(a)
\begin{lemm}
    Let $\bzeta = [\zeta_1,\ldots,\zeta_n]$ be a $L$-sub-exponential MDS and let $T \in \R^n, n \geq 2$. Then, for every $p \geq 1$,
    \begin{align}
        \left( E \sup_{t \in T} | \langle t, \bzeta \rangle |^p \right)^{1/p} & \leq c_2 \left( \sqrt{\log n} \cdot E \left[ \sup_{t \in T} | \langle t, \bgg \rangle | \right] + \sup_{t \in T} \left( E| \langle t, \bzeta \rangle|^p \right)^{1/p} \right)~ 
    \end{align}
    where $c_2$ is a constant which depends on $L$, $\bgg = [g_j]$ where $g_j$ are independent identically distributed normal random variables, and
    $\eta = [\eta_j]$ where $\eta_j$ are independent identically distributed exponential random variables.
    % \begin{align}
    %     \left( E \sup_{t \in T} | \langle t, \bzeta \rangle |^p \right)^{1/p} & \leq c_2 \left( E \left[ \sup_{t \in T} | \langle t, \bgg \rangle | \right] + E \left[ \sup_{t \in T} | \langle t, \beeta \rangle | \right] + \sup_{t \in T} \left( E| \langle t, \bzeta \rangle|^p \right)^{1/p} \right)~ 
    % \end{align}(a)
    % where $c_2$ is a constant which depends on $L$, $\bgg = [g_j]$ where $g_j$ are independent identically distributed normal random variables, and
    % $\eta = [\eta_j]$ where $\eta_j$ are independent identically distributed exponential random variables.
\label{lemm:lpnorme}
\end{lemm}

We need the following basic property of sub-exponential random variables to prove Lemma~\ref{lemm:lpnorme}.
\begin{prop}
If $X$ is a $L$-sub-exponential random variable, then
\begin{equation}
     P(|X| > t L) \leq 2 \exp(-t)~, ~~\forall t \geq 0 \qquad \Leftrightarrow \qquad  (E|X|^p)^{1/p} \leq c_0 p L~, ~~\forall p~. 
 \end{equation}
\label{prop:sube}
\end{prop}

We also need the following result on mixed tails:
\begin{prop}
Consider a random variable $X$ such that
\begin{equation}
     P(|X| > \sqrt{t} L_2 + tL_1) \leq 2 \exp(-t)~, ~~\forall t \geq 0~.  
 \end{equation}
Then
\begin{equation}
    (E|X|^p)^{1/p} \leq c_0 \sqrt{p} L_2 + p L_1~, ~~\forall p \geq 1~. 
\end{equation}
\label{prop:sube2}
\end{prop}
\proof Note that for $\sqrt{t} L_1 \leq t L_1$, we have 
\begin{align*}
    P(|X| > 2 \sqrt{t} L_2 ) & \leq P(|X| > \sqrt{t} L_2 + tL_1)  \leq 2 \exp(-t) \\
\Rightarrow \quad P(|X| > t ) & \leq 2 \exp(-t^2/4L_2^2)~.
\end{align*}
For $\sqrt{t} L_1 \geq t L_1$, we have
\begin{align*}
    P(|X| > 2 t L_1 ) & \leq P(|X| > \sqrt{t} L_2 + tL_1) \leq 2 \exp(-t) \\
\Rightarrow \quad P(|X| > t ) & \leq 2 \exp(-t/2L_1)~.
\end{align*}
Hence, for all $t \geq 0$
\begin{equation}
    P(|X| > t ) \leq 2 \exp(-\min(t^2/4L_2^2, t/2L_1))~.
\end{equation}
Now, recall that for any non-negative random variable $E[Z] = \int_0^{\infty} P(Z \geq u) du$. Using $Z=|X|^p, u = t^p$, we have
\begin{align*}
    E|X|^p & = \int_0^{\infty} P(|X| > t) p t^{p-1} dt \\
    & \leq \underbrace{2 \int_0^{\infty}  \exp(-t^2/4L_2^2) p t^{p-1} dt}_{\cI_1} + \underbrace{2 \int_0^{\infty} \exp(-t/2L_1) p t^{p-1} dt}_{\cI_2}~.
\end{align*}
For the first term $\cI_1$, consider change of variables $t_2 = t/2L_2$, so $dt = 2 L_2 dt_2$ to give
\begin{align*}
    \cI_1 = 2 \cdot 2^p L_2^p p \int_0^{\infty} \exp(-t_2^2) t_2^{p-1} dt_2 \leq 2 c_2^p L_2^p p (p)^{p/2}~, 
\end{align*}
for a suitable constant $c_2$, following Proposition~\ref{prop:subg}~\cite{vers12}.
For the second term $\cI_2$, consider change of variables $t_1 = t/2L_1$, so $dt = 2L_1 dt_1$ to give
\begin{align*}
    \cI_2 = 2 \cdot 2^p L_1^p p \int_0^{\infty} \exp(-t_1) t_1^{p-1} dt_1 \leq 2 c_1^p L_1^p p (p)^{p}~, 
\end{align*}
for a suitable constant $c_1$, following Proposition~\ref{prop:sube}~\cite{vers12}. Taking $p$-th roots and using Jensen's inqeaulity, we have
\begin{align*}
    (E|X|^p)^{1/p} & \leq (\cI_1)^{1/p} + (\cI_2)^{1/p}  \leq c_0 ( \sqrt{p} L_2 + p L_1)~,
\end{align*}
for a suitable constant $c_0 >0 $. That completes the proof. \qed


% {\bf notes} We develop a basic tail bound of $L_p$ norm of sub-Gaussian random variables. Note that for $u \geq c_0$, if
% \[
% P(X > u) \leq 2 \exp(- c_1 u^2 p)~, 
% \]
% we have
% \begin{align*}
% \int_{c_0}^{\infty} p u^{p-1} P(X > u) du & \leq 2 \int_{c_0}^{\infty} p u^{p-1} \exp(-c_1 u^2 p) du~.
% \end{align*}
% Consider the change of variables $t = u \sqrt{p}$, so that $du = \frac{1}{\sqrt{p}} dt$. Then,
% \begin{align*}
% \int_{c_0}^{\infty} p u^{p-1} P(X > u) du & \leq 2 \int_{c_0 \sqrt{p}}^{\infty} \sqrt{p} t^{p-1} p^{-(p-1)/2} \exp(-c_1 t^2 ) dt \leq \sqrt{p} \kappa_2^{p-1}~,
% \end{align*}
% where $\kappa_2$ is the $\psi_2$-norm. 

% {\bf Proposition.} We also develop a basic tail bound of $L_p$ norm of sub-exponential random variables. Note that for $u \geq c_0$, if
% \[
% P(X > u) \leq 2 \exp(- c_1 u p)~, 
% \]
% we have
% \begin{align*}
% \int_{c_0}^{\infty} p u^{p-1} P(X > u) du & \leq 2 \int_{c_0}^{\infty} p u^{p-1} \exp(-c_1 u p) du~.
% \end{align*}
% Consider the change of variables $t = u p$, so that $du = \frac{1}{p} dt$. Then,
% \begin{align*}
% \int_{c_0}^{\infty} p u^{p-1} P(X > u) du & \leq 2 \int_{c_0 \sqrt{p}}^{\infty} t^{p-1} p^{-(p-1)} \exp(-c_1 t ) dt \leq \kappa_1^{p-1}~,
% \end{align*}
% where $\kappa_2$ is the $\psi_2$-norm.

We also need the following result from~\cite{sibp15}:
\begin{theo}
For any $T \subset \R^n$, we have 
\begin{equation}
    E\left[\sup_{t \in T}|\langle t, \beeta \rangle|\right] \leq \sqrt{\log n} \cdot E\left[\sup_{t \in T}|\langle t, \bgg \rangle|\right]~,
\end{equation}
where $\bgg = [g_j]$ where $g_j$ are independent identically distributed normal random variables, and
    $\beeta = [\eta_j]$ where $\eta_j$ are independent identically distributed exponential random variables.
\label{theo:exp-width}
\end{theo}



{\em Proof of Lemma~\ref{lemm:lpnorme}.} We assume $T$ is finite without loss of generality. Let $\{T_r\}$ be an optimal admissible sequence of $T$. For any $t \in T$, let $\pi_r(t) = \argmin_{t_r \in T_r} \| t - t_r\|_2$. For any given $p$ determining the $p$-norm, choose $\ell$ such that $2^{\ell-1} \leq 2p \leq 2^{\ell}$, so that $2^{\ell} / p \leq 4$. Then, by triangle inequality, we have
\begin{equation}
    \sup_{t \in T}|\langle t,\bzeta \rangle| \leq \sup_{t \in T} | \langle \pi_{\ell}(t), \bzeta \rangle | + \sup_{t\in T} \sum_{r=\ell}^{\infty} | \langle \pi_{r+1}(t) - \pi_r(t), \bzeta \rangle |~.
\end{equation}
For the first term, note that
\begin{align*}
    \left( E \sup_{t \in T} | \langle \pi_{\ell}(t), \bzeta \rangle |^p \right)^{1/p} 
    & \leq \left( E \sum_{t \in T_{\ell}} | \langle t, \bzeta \rangle |^p \right)^{1/p} \\
    & \leq (|T_{\ell}|)^{1/p} \sup_{t \in T_{\ell}} \left(E| \langle t, \bzeta \rangle |^p \right)^{1/p} \\
    & \leq (2^{2^{\ell}})^{1/p} \sup_{t \in T} (E|\langle t,\bzeta \rangle|^p)^{1/p} \\
    & \leq 16 \sup_{t \in T} (E|\langle t,\bzeta \rangle|^p)^{1/p}~.
\end{align*}
% we first define the following function:
% \begin{align}
%     f(u, r, t, t', \{x_j\}) = \begin{cases}
%     u L_2 2^{r/2} \| (\langle \pi_{r+1}(t) - \pi_r(t), x_j \rangle)_{j=1}^n \|_2~, & ~~\text{if}~~ u \leq L_2^2/L_1~, \\
%     u L_{\infty} 2^{r} \| (\langle \pi_{r+1}(t) - \pi_r(t), x_j \rangle)_{j=1}^n \|_{\infty}~, & ~~ \text{otherwise}~.
%     \end{cases}
% \end{align}
For the second term, for any $u \geq 0$, we have 
\begin{align*}
    P & \bigg( \sup_{t\in T} \sum_{r=\ell}^{\infty} | \langle \pi_{r+1}(t) - \pi_r(t), \bzeta \rangle | 
    \geq  \sqrt{u} L 2^{r/2} \|  \pi_{r+1}(t) - \pi_r(t) \|_2  \\
    & \phantom{...................................................}
    + u L 2^{r} \|  \pi_{r+1}(t) - \pi_r(t) \|_{\infty}   \bigg)  \\
    & \leq \sum_{t=\ell}^{\infty} \sum_{t \in T_{r+1}} \sum_{t' \in T_r} P \bigg( \bigg| \langle t - t', \bzeta \rangle \bigg| \geq \sqrt{u} L 2^{r/2} \| t - t' \|_2  \\
    &  \phantom{......................................................} 
    + u L 2^{r} \| t - t' \|_{\infty} \bigg) \\
    & \stackrel{(a)}{\leq} \sum_{r=\ell}^{\infty} 2^{2^{r+1}} \cdot 2^{2^r} \cdot \exp (-2^{r} u) 
    \leq 2 \exp(- 2^{\ell} u) \\
    & \leq 2 \exp(-p u)~,
\end{align*}
for $u \geq u_0$, a constant, and where (a) follows from the Azuma-Bernstein inequality. 

Then, from Proposition~\ref{prop:sube2}, we have
\begin{align*}
    \left( E \sup_{t\in T} \sum_{r=\ell}^{\infty} | \langle \pi_{r+1}(t) - \pi_r(t), \bzeta \rangle |^p \right)^{1/p} 
    & \leq L \sum_{r=\ell}^{\infty} \bigg( 2^{r/2} \| \pi_{r+1}(t) - \pi_r(t) \|_2  \\
    & \phantom{..............} +   2^{r} \|  \pi_{r+1}(t) - \pi_r(t) \|_{\infty} \bigg) \\
    & \leq L (\gamma_2(T, \| \cdot \|_2) + \gamma_1(T, \| \cdot \|_{\infty} )~.
\end{align*}
% where $T' = \{ (\langle t, x_j \rangle)_{j=1}^n | t \in T \}$. 
Then, by the majorizing measures theorem [][], we have
\begin{equation*}
     \gamma_2(T,\| \cdot \|_2 ) \leq E \sup_{t \in T} |  \langle t, \bgg \rangle |~, \quad \text{and} \quad  
        \gamma_1(T,\| \cdot \|_{\infty} ) \leq E \sup_{t \in T} |  \langle t, \beeta \rangle | \stackrel{(a)}{\leq} \sqrt{\log n}  \cdot  E \sup_{t \in T} |  \langle t, \bgg \rangle |~
\end{equation*}
% and 
% \begin{equation*}
%     \gamma_1(T',\| \cdot \|_{\infty} ) \leq E \sup_{t' \in T'} \left| \langle t', \eta \rangle \right| 
%     = E \sup_{t \in T} \left| \sum_{j=1}^n \langle t, x_j \rangle \eta_j \right| = E \sup_{t \in T} |  \langle t, \eta \rangle |~. 
% \end{equation*}
where (a) follows from Theorem~\ref{theo:exp-width}. Noting that $(1+ \sqrt{\log n}) \leq 3 \sqrt{\log n}$ for $n \geq 2$ completes the proof. \qed


%\ab{Proof of Theorem~\ref{theo:subg-diag} can be now be done using Lemma~\ref{lemm:lpnorme}.}

{\em Proof of Theorem~\ref{theo:subg-diag}.} Consider the random variable $\bzeta^{(A)} = \sum_{j=1}^n (\xi^2 - E|\xi_j|^2) \| A^j \|_2^2$. Then, for any $A,B \in \cA$, by Azuma-Bernstein inequality, we have
\begin{equation}
    P\left( | \bzeta^{(A)} - \bzeta^{(B)} | \geq \eps\right) \leq 2 \exp \left\{ -\min \left( \frac{\eps^2}{d_2^2(A,B)}, \frac{\eps}{d_1(A,B)} \right) \right\}~, 
\end{equation}
where
\begin{align*}
    d_2(A,B) &= ~ \left( \sum_{j=1}^n (\| A^j \|_2^2 - \| B^j \|_2^2 )^2 \right)^{1/2} \\ 
    & = ~ \left( \sum_{j=1}^n ( \| A^j \|_2 - \| B^j \|_2 )^2 \cdot (\| A^j \|_2 + \| B^j \|_2 )^2 \right)^{1/2} \\
    & \stackrel{(a)}{\leq} ~ \left( \sum_{j=1}^n \| A^j - B^j \|_2^2 \cdot (\| A^j \|_2 + \| B^j \|_2 )^2 \right)^{1/2} \\
    & \leq ~ 2 d_F(\cA) \| A - B \|_{2 \rightarrow 2}~,
\end{align*}
where (a) follows from triangle inequality, and 
\begin{align*}
    d_1(A,B) & = ~ \left\| \| A^j \|_2^2 - \| B^j \|_2^2 \right\|_{\infty} \\
    & = ~ \left\| (\| A^j \|_2 - \| B^j \|_2) (\|A^j \|_2 + \| B^j \|_2) \right\|_{\infty} \\
    & \stackrel{(a)}{\leq} ~ 2d_F(\cA) \left\| \| A^j - B^j \|_2 \right\|_{\infty} \\
    & = d_F(\cA) \| A - B\|_{2,\infty}~,
\end{align*}
where (a) follows from triangle inequality. Also, recall from the majorizing measure theorem that
$E[\sup_{t \in T}|\langle t, \bgg \rangle|] \leq \gamma_2(T, d_2)$.
Then, from Lemma~\ref{lemm:lpnorme} and Proposition~\ref{prop:sube2}, we have
\begin{align*}
 \| D_{\cA}(\bxi) \|_{L_p} 
 %& \leq E[\sup_{t \in T}|\langle t, \bgg \rangle|] + E[\sup_{t \in T}|\langle t, \beeta \rangle|] + \sup_{t \in T}~ (E|\langle t, \bzeta \rangle |^p )^{1/p} \\
%  & \leq (1+ \sqrt{\log n}) E[\sup_{t \in T}|\langle t, \bgg \rangle|] + \sup_{t \in T}~ (E|\langle t, \bzeta \rangle |^p )^{1/p} \\
  & \leq \sqrt{\log n} \cdot d_F(\cA) \cdot \gamma_2(  \cA, \| \cdot \|_{2 \rightarrow 2} ) + \sqrt{p} \cdot d_F(\cA) \cdot d_{2 \rightarrow  2} + p \cdot d_F(\cA) \cdot d_{2,\infty}(\cA)~.
\end{align*}
% where 
% %(a) follows from Theorem~\ref{theo:exp-width} and 
% (b) follows from the majorizing measures theorem [][]. Further, from Proposition~\ref{prop:sube2}, we have 
% \begin{align*}
%     \sup_{t \in T}~ (E|\langle t, \bzeta \rangle |^p )^{1/p} & =     \sup_{A \in \cA}~ (E|\sum_{j=1}^n \| A^j \|_2^2 \zeta_j |^p )^{1/p} \\
%     & \stackrel{(a)}{\leq} \sqrt{p} \sup_{A \in \cA} \| A \|_F + p \sup_{A \in \cA} \| A \|_{2,\infty} \\
%     & = \sqrt{p} \cdot d_F(\cA) + p \cdot d_{2,\infty}(\cA)~.
% \end{align*}
That completes the proof. \qed



==> sec/proofs-main.tex <==

With the existing bounds on the $L_p$ norms of the off-diagonal and diagonal terms from Section~\ref{ssec:subg-main}, the proofs of the main results, Theorem 1 and Theorem 2, follow from  \eqref{eq:lpp1}-\eqref{eq:lpp3}.

{\em Proof of Theorem 1:} For bounded random variables, the main result follows by combining the off-diagonal $L_p$ norm bound in Theorem~~\ref{theo:offd} and the diagonal $L_p$ norm bound in Theorem~\ref{theo:subg-diag-bnd} and \eqref{eq:lpp1}-\eqref{eq:lpp3}. \qed


{\em Proof of Theorem 2:} For unbounded sub-Gaussian random variables, the main result follows by combining the off-diagonal $L_p$ norm bound in Theorem~~\ref{theo:offd} and the diagonal $L_p$ norm bound in Theorem~\ref{theo:subg-diag} and \eqref{eq:lpp1}-\eqref{eq:lpp3}. \qed



==> sec/rip-rademacher.tex <==

Let $\xi_1,\ldots,\xi_n$ be a Rademacher martingale difference sequence (MDS) so that
\beq 
E[\xi_i|\cF_{i-1}] = 
\begin{cases}
+1~,  & ~~\text{with probability}~~ \frac{1}{2}~,\\
-1~,  & ~~\text{with probability}~~ \frac{1}{2}~.
\end{cases}
\eeq

\begin{theo}
Let $\cA \subset \R^{m \times n}$ be a collection of $(m \times n)$ matrices. Let $\xi_1,\ldots,\xi_n$ be a Rademacher MDS, and
let $\xi \in \R^n$ denote a vector of these random variables.
Then,
\beq
E_{\xi} \sup_{A \in \cA} \left| \| A \xi \|^2 - E \| A \xi \|^2 \right| \leq \gamma_2^2(\cA, \| \cdot \|) + \gamma_2(\cA,\| \cdot \|) \cdot d_F(\cA) + d_{2 \rightarrow 2}(\cA) \cdot d_F(\cA)~,
\eeq
where $d_X(T)$ denotes the diameter of $T$ w.r.t.~norm $\|\cdot\|_X$, $X =F$ denotes the Frobenius norm and $X = 2 \rightarrow 2$
denotes the operator norm.
\end{theo}
Our analysis is based on a generalization of the main result in \cite{krmr14} for i.i.d.~random variables to MDS.
The analysis is based generic chaining and needs the following key definition due to Talagrand~\cite{tala14}.
\begin{defn}
For a metric space $(T,d)$, an admissible sequence of $T$ is a collection of subsets of $T$, $\{T_r : r \geq 0\}$,
with $|T_0| = 1$ and $|T_r| \leq 2^{2^r}$ for all $r \geq 1$. For $\beta \geq 1$, the $\gamma_{\beta}$ functional is defined by
\beq
\gamma_{\beta}(T,d) = \inf \sup_{t \in T} \sum_{r=0}^{\infty} 2^{r/\beta} d(t,T_r)~,
\eeq
where the infimum is over all admissible sequences of $T$.
\end{defn}


\proof Without loss of generality, assume $\cA$ is finite. Let 
\beq
\Gamma = E_{\xi} \sup_{A \in \cA} \left| \| A \xi \|^2 - E \| A \xi \|^2 \right|~.
\eeq
Using the fact that $\xi$ is a Rademacher MDS so that the diagonal canecls out and using Theorem~\ref{th:mds-dec}, if $A_j, j \in [n]$ denote the $j^{th}$  column of $A$, we have
\begin{align*}
\Gamma & = E_{\xi} \sup_{A \in \cA} \left| \sum_{j \neq k} \xi_j \xi_k \langle A_j, A_k \rangle \right|  \leq E_{\xi,\xi'} \sup_{A \in \cA} \left| \sum_{j \neq k} \xi_j \xi'_k \langle A_j, A_k \rangle \right|  = E_{\xi,\xi'} \sup_{A \in \cA} \left|  \langle A \xi, A \xi' \rangle \right|~,
\end{align*}
where $\xi'$ corresponds to a decoupled tangent sequence to $\xi$. 

Let $\{T_r\}_{r=0}^{\infty}$ be an admissible sequence for $\cA$ for which the minimum in the definition
of $\gamma_2(\cA, \| \cdot \|_{2 \rightarrow 2})$ is attained. Let 
\beq
\pi_r A = d_{2 \rightarrow 2}(A,T_r) = \underset{B \in T_r}{\argmin} ~\| B - A\|_{2 \rightarrow 2} \qquad \text{and} \qquad \Delta_r A = \pi_r A - \pi_{r-1} A~.
\eeq
Then, by a direct computation based on a telescoping sum, we have 
\beq
\langle A \xi, A \xi'\rangle = \langle (\pi_0 A) \xi, (\pi_0 A) \xi' \rangle 
+ \sum_{r=1}^{\infty} \langle (\Delta_r A) \xi, (\pi_{r-1} A) \xi' \rangle 
+ \sum_{r=1}^{\infty} \langle (\pi_r A) \xi, (\Delta_{r-1} A) \xi' \rangle~. 
\eeq
Since we have $T_0 = \{ A_0 \}$ for some $A_0 \in \cA$, we have $\pi_0 A = A_0$, so that
\begin{align*}
E_{\xi,\xi'} \left| \langle (\pi_0 A) \xi, (\pi_0 A) \xi' \rangle \right| 
& = E_{\xi,\xi'} \left| \xi^T A_0^T A_0 \xi' \right| \\
& \leq \left( E_{\xi,\xi'} \left| \xi^T A_0^T A_0 \xi' \right)^{1/2} = \| A_0^T A_0 \|_F \\
& \leq \| A_0 \|_F \| A_0 \| 
\leq d_F(\cA) \cdot d_{2 \rightarrow 2}(\cA)~.
\end{align*}
Hence, 
\beq
E_{\xi,\xi'} \sup_{A \in \cA} \left| \langle A \xi, A \xi' \rangle \right| 
\leq d_F(\cA) \cdot d_{2 \rightarrow 2}(\cA)
+ E_{\xi,\xi'} \sup_{A \in \cA} \sum_{r=1}^{\infty} \left| X_r(A) \right|   
+ E_{\xi,\xi'} \sup_{A \in \cA} \sum_{r=1}^{\infty} \left| Y_r(A) \right|~,
\label{eq:cbnd1}
\eeq
where
\begin{align}
X_r(A)  & = \langle (\Delta_r A) \xi, (\pi_{r-1} A) \xi' \rangle~,  \\
Y_r(A)  & = \langle (\pi_r A) \xi, (\Delta_{r-1} A) \xi' \rangle~.
\end{align}
Conditioning $X_r$ on $\xi'$, we note
\beq
X_r(A) = \langle (\Delta_r A) \xi, (\pi_{r-1} A) \xi' \rangle = \langle  \xi, (\Delta_r A)^T (\pi_{r-1} A) \xi' \rangle~,
\eeq
which is a weighted sum of a MDS. Then, a direct application of the Azuma-Hoeffding bound gives
\beq
P\left( |X_r(A) | > u \| (\Delta_r A)^T (\pi_{r-1} A) \xi' \| ~\bigg| ~\xi' \right) \leq 2 \exp(-u^2/2)~.
\eeq
Using $u = t 2^{r/2}$, we get
\beq
P\left( |X_r(A) | > t 2^{r/2} \| (\Delta_r A)^T (\pi_{r-1} A) \xi' \| ~\bigg|~ \xi' \right) \leq 2 \exp(-t^2 2^r/2)~.
\label{eq:azho}
\eeq
Since
\beq
\left| (\Delta_r A)^T (\pi_{r-1} A) \xi' \right| 
\leq \| \Delta_r A \|_{2 \rightarrow 2} \sup_{A \in \cA} \| A \xi' \|_2~.
\eeq
we have 
\beq
P\left( |X_r(A) | > t 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2} \sup_{A \in \cA} \| A \xi' \|_2 ~\bigg|~ \xi' \right) \leq 2 \exp(-t^2 2^r/2)~.
\eeq
Now, by union bound, we get 
\begin{align}
P\left( \sup_{A \in \cA} \sum_{r=1}^{\infty} |X_r(A)| > t \left(\sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2} \right) \cdot \sup_{A \in \cA} \| A \xi' \|_2 ~\bigg|~ \xi' \right)  
& \leq 2 \sum_{r=1}^{\infty} |T_r| \cdot |T_{r-1}| \cdot \exp(-t^2 2^r/2) \\
& \leq 2 \sum_{r=1}^{\infty} 2^{2^{r+1}} \cdot \exp (-t^2 2^r/2)~. \label{eq:bnd42}
\end{align}
We focus on upper bounding the second term in \eqref{eq:cbnd1}, noting that the third term can be similarly bounded.
First, note that
\beq
E_{\xi,\xi'} \sup_{A \in \cA} \sum_{r=1}^{\infty} | X_r(A) | = E_{\xi'} \int_0^{\infty} P_{\xi}\left( \sup_{A \in \cA} \sum_{r=1}^{\infty} |X_r(A)| > \tau ~\bigg|~\xi' \right) d\tau~.
\eeq
Let
\begin{align*}
    \tau & = t  \sup_{A \in \cA} \| A \xi' \|_2 \cdot \left(\sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2}\right)  \\
    \Rightarrow \qquad d\tau & =  \sup_{A \in \cA} \| A \xi' \|_2 \cdot \left( \sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2} \right)  dt~.
\end{align*}
With this change of variables, we have 
\begin{align*}
E_{\xi,\xi'} \sup_{A \in \cA}  \sum_{r=1}^{\infty} | X_r(A) | & = E_{\xi'} \left[
\sup_{A \in \cA} \| A \xi' \|_2 \cdot \left( \sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2} \right) \right.  \\
& \phantom{...........} \times \left. \int_0^{\infty} P_{\xi} \left( \sup_{A \in \cA} \sum_{r=1}^{\infty} |X_r(A)| > t \left(\sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2} \right) \cdot \sup_{A \in \cA} \| A \xi' \|_2 ~\bigg|~\xi' \right) dt \right] \\
& \stackrel{(a)}{\leq} E_{\xi'} \left[\sup_{A \in \cA} \| A \xi' \|_2 \right] \cdot \left( \sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2} \right) \cdot \left( 4 + 2 \sum_{r=1}^{\infty} 2^{2^{r+1}} \cdot \int_4^{\infty}  \exp(-t^2 2^r/2) dt  \right) \\
& \stackrel{(b)}{\leq} 5 E_{\xi'} \left[\sup_{A \in \cA} \| A \xi' \|_2 \right] \cdot \left( \sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} \| \Delta_r A \|_{2 \rightarrow 2} \right) \\
& \stackrel{(c)}{\leq} 10 E_{\xi'} \left[\sup_{A \in \cA} \| A \xi' \|_2 \right] \cdot \left( \sup_{A \in \cA} \sum_{r=1}^{\infty} 2^{r/2} d_{2 \rightarrow 2}(A,T_r) \right) ~,
\end{align*}
where (a) follows from an application of \eqref{eq:bnd42}, (b) follows by directly bounding the last term using Gaussian integrals\footnote{Show the details, but this is straightforward.}, and (c) follows by triangle inequality since 
\begin{equation*}
    \| \Delta_r A \|_{2 \rightarrow 2} \leq d_{2 \rightarrow 2}(A,T_{r-1}) + d_{2 \rightarrow 2}(A,T_r)~. 
\end{equation*}
Choosing an admissible sequence $\{T_r\}$  to minimize the upper bound, by definition of Talagrand's $\gamma$-function we have
\begin{equation*}
    E_{\xi,\xi'} \sup_{A \in \cA}  \sum_{r=1}^{\infty} | X_r(A) |  
    \leq 10 E_{\xi'} \left[\sup_{A \in \cA} \| A \xi' \|_2 \right] \gamma_2(\cA, \| \cdot \|_{2 \rightarrow 2})~.
\end{equation*}
Plugging this back in \eqref{eq:cbnd1} and noting that the third term in \eqref{eq:cbnd1} can be similarly bounded, we have
\begin{equation}
    \Gamma = E_{\xi,\xi'} \sup_{A \in \cA} \left| \langle A \xi, A \xi' \rangle \right| 
\leq d_F(\cA) \cdot d_{2 \rightarrow 2}(\cA) + 20 E_{\xi'} \left[\sup_{A \in \cA} \| A \xi' \|_2 \right] \gamma_2(\cA, \| \cdot \|_{2 \rightarrow 2})~.
\label{eq:cbnd2}
\end{equation}
Now, by Jensen's inequality
\begin{align*}
    E_{\xi'} \left[\sup_{A \in \cA} \| A \xi' \|_2 \right] 
&    \leq \left( E_{\xi'} \left[\sup_{A \in \cA} \| A \xi' \|^2_2 \right] \right)^{1/2} \\
&    \leq \left( E_{\xi'} \left[\sup_{A \in \cA} \left\{ \left| \| A \xi' \|^2_2 
    - E_{xi'} \| A \xi' \|_2^2 \right| + E_{\xi'} \| A \xi' \|_2^2 \right\} \right] \right)^{1/2} \\
&   =  \left( E_{\xi'} \left[\sup_{A \in \cA} \left\{ \left| \| A \xi' \|^2_2 
    - E_{xi'} \| A \xi' \|_2^2 \right| + \| A \|_F^2 \right\} \right] \right)^{1/2} \\
& \leq \sqrt{\Gamma} + d_F(\cA)~.
\end{align*}
Then, from \eqref{eq:cbnd2}, we get
\begin{align}
    \Gamma & \leq d_F(\cA) \cdot d_{2 \rightarrow 2}(\cA) + 20 (\sqrt{\Gamma} + d_F(\cA)) \gamma_2(\cA, \| \cdot \|_{2 \rightarrow 2})~. 
\end{align}
The main result follows by solving the quadratic inequality for $\Gamma$. \qed


==> sec/sketch.tex <==

This is the sketch of the analysis.
